What is in Your Safe Data? Identifying Benign Data that Breaks Safety

Current Large Language Models (LLMs), even those tuned for safety and alignment, are susceptible to jailbreaking. Some have found that just further fine-tuning an aligned model with benign data (i.e., data without harmful content) surprisingly leads to substantial degradation in safety. We delve into the data-centric aspects of why benign fine-tuning inadvertently contributes to jailbreaking. First, we represent fine-tuning data through two lenses: representation and gradient spaces. Additionally, we propose a bi-directional anchoring method that, during the selection process, prioritizes data points that are close to harmful examples and far from benign ones. Our approach effectively identifies subsets of benign data that are more likely to degrade the model's safety after fine-tuning. Training on just 100 of these seemingly benign datapoints surprisingly leads to the fine-tuned model affirmatively responding to >70% of tested harmful requests, compared to <20% after fine-tuning on randomly selected data. We also observe that the selected data frequently appear as lists, bullet points, or math questions, indicating a systematic pattern in fine-tuning data that contributes to jailbreaking.

==> tables/harmful_anchoring.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{0.3}
    \begin{tabular}{lcccc}
    \toprule
\textbf{Harmful Example Type}    & \textbf{Selection Type} & \textbf{  Keyword ASR  } & \textbf{ 
 GPT Score  } & \textbf{  GPT ASR  } \\ \cmidrule(r){1-5} \\
Illegal activities  &  Top 100 & 95.19\% & 3.81  & 66.54\%\\
&  Bottom 100 & 5.58\% & 1.14  & 1.73\%\\
 \cmidrule(r){1-5} \\
Hate Speech  &  Top 100 & 86.15\% & 3.40  & 54.00\%\\
 &  Bottom 100 & 19.04\% & 1.30 & 6.00\%\\
    \bottomrule
    \end{tabular}
    \caption{Effectiveness of using few examples of same harmfulness category as $\dharmful$}
    \label{tab:harmful_anchor}
\end{table}

